A cylindrical GEM detector for BES III

BESIII is a particle physics experiment located at the Institute of High-Energy Physics (BEPC-II) e+e- collider at IHEP in Beijing. The Italian collaboration is leading the effort for the development of a cylindrical GEM (CGEM) detector with analog readout to upgrade the current inner drift chamber that is suffering early ageing due to the increase of the machine luminosity. Within the CGEM project, this work aims to perform full detector simulation for the optimisation of the tracker geometry and its operational parameters. The goal is achieved by means of three different, but well connected, studies: a background estimation, a simulation of the detection elements and the data analysis of a beam test. I participated to the construction of the cathode electrode, that was produced in Ferrara, helping during the assembling and manufacturing procedures. For the background studies and the detector simulation I took care both of the framework development and of the data analysis. Finally, I participated to installation and data taking of the beam test at CERN, and I was involved in the production of the reconstruction and analysis software. During and after the beam test I participated to the processing and analysis of the data.

==> Chapter1_troppolungo.tex <==
QUEL CHE ERA IL CAPITOLO 1

\section{The Physics program}
\label{sec:physics}

The BESIII physics plan is to accumulate a significant data sample of charmonium states for high precision measurements: $e.g.$ $10^{10}$ J/$\Psi$, $10^9$ $\Psi$(2S), $10^6$ D$\overline{D}$.
The aim is to be sensitive to new physics observation concerning hot topics like $D^0\overline{D^0}$ mixing, the charmonium-like XYZ states and CP violation in charmed-quark and $\tau$ sector.
The high precision measurements at BESIII are compared with QCD calculations. The huge data sample allows to search for rare decays like lepton-number violation or flavour violating processes.

\subsection{Hadrons Spectroscopy}
BESIII investigates the structure of matter and the nature of the interactions between its constituent components \cite{BesIIIphysicsbook}. 
To access  a smaller object it occurs to increase the energy scale but increasing the energy changes the theoretical description of the phenomena. 
At momentum transfers around the MeV scale, below $\Lambda_{QCD}$ $\sim$ 200 MeV the fundamental scale of Quantum Chromodynamics {QCD}, the chiral symmetry theory can provide solutions to study the low-energy dynamics as QCD becomes non-perturbative \cite{Brambilla}. 

Increasing more the energy in a range that is greater than $\Lambda_{QCD}$ partonic and gluonic behaviour is shown in the deep inelastic scattering. In this energy region it is allow to study QCD process through perturvative expansion \cite{Brambilla}. 
In the region between these two energy scales there is no theory that can describe the phenomena so meson and baryon resonances are studied to know the constituent behaviour. 

These pieces compose the QCD puzzle and the hadrons spectroscopy plays an important role in its interpretetion.
In the light quark sector ($u, d, s$) the mass differences are relatively small: $m_u$ $\sim$ 3 MeV, $m_d$ $\sim$ 5 Mev and $m_s$ $\sim$ 95 MeV \cite{ChinesePhysicsC} then the strong interaction can be approximate with a global SU(3) flavour symmetry. This approach allows to predict the hadrons masses of mesons and baryons composed by the quarks of the symmetry. Different regimes and their validity range are summarized in Tab. $\ref{table:Teories}$ 

The QCD calculation in this region are described by these hypotheses with a naïve quark model \cite{Isgur,KTChao}:
\begin{itemize}
\item spontaneous breaking of chiral symmetry leads to the presence of massive constituent
quarks within a hadron as effective degrees of freedom.
\item hadrons can be viewed as a quark system in which the gluon fields generate effective
potentials that depend on the relative positions and spins of the massive quarks.
\end{itemize}

\begin{table}[ht]
\begin{minipage}{\textwidth}
\begin{center}
\begin{tabular}{l|lc}
\hline
Theory Name     & Energy Scale        &       \\
\hline
The chiral-symmetry theory 	& 	E < $\Lambda_{QCD}$ 	& 	\\
Perturbative QCD		&	E >>$\Lambda_{QCD}$	&	\\
Global SU(3) flavour symmetry	&	E < $\Lambda_{QCD}$	&	\\
Non-relativistic QCD		&	E > 1 GeV		&	\\
\hline
\end{tabular}
\caption[Theories and energy scale.]{Different theory used and their energy scale validity.}
\label{table:Teories}
\end{center}
\end{minipage}
\end{table}

A non-relativistic approach can be used with the naïve method for quarks that have constituent masses comparable or greater than the $\Lambda_{QCD}$. For quarks with an excitation energy of the excited hadrons states comparable to their masses this approach has no sense but it works in a wide range of empirical test \cite{Brambilla}. 

Several theoris can be found in literature: the semirelativistic flux-tube model \cite{Carlson,Sartor}, the instanton model \cite{Blask}, the Goldstone boson exchange model \cite{Glozman}, the diquark model \cite{Anselmino}, etc.

The ultimate goal of the study of the hadron spectroscopy is to understand the dynamics of the constituent interactions. Conventional $q\overline{q}$ meson can be constructed in the quark model and their spectrum is studied to be described in an exmpirically efficient way. QCD also allows the existence of other bound states that are made completely of gluons ($e.g.$ so called “glueball”), multiquark mesons, such as $qq\overline{qq}$ and so-called “hybrid” mesons which contain both $q\overline{q}$ and gluon.
Glueballs are bound states of at least 2 or 3 gluons in a color singlet. Assuming that gluons inside glueballs are massive, for $gg$ with angular momentul L = 0, states of $J^{PC}$ = $0^{++}$ and $2^{++}$. For $ggg$ the lowest states are $0^{-+}$, $1^{--}$ and $3^{--}$.
Both $gg$ and $ggg$ can form states with quantum number that cannot be produced by $q\overline{q}$ states.

	\begin{figure}[hbtp]
		\centering
   		\includegraphics[width=0.7\textwidth]{figure/GlueballSpectrum.pdf}
   		\caption[Glueball spectrum.]{Glueball Spectrum. Glueball states are labeled by J$^{PC}$, where J is the spin quantum number and P and C are parity and charge conjugation, respectively.}
	\label{fig:fgGlueball}
	\end{figure}

The abundance of isoscalar scalars in the 1-2 GeV, mass region, $e.g.$ the $f_0$(1370), $f_0$(1500), and $f_0$(1710) (the $f_0$(1790) and $f_0$(1810) should be confirmed in further experiments), makes them natural scalar glueball candidates and they are studied at BESIII as decay products. Hybrid mesons are hypothesized to be formed from a $q\overline{q}$ pair plus one explicit gluon field. Evidence for the existence of hybrid mesons would be direct proof of the existence of the gluonic degree of freedom and the validity of QCD. In addition, the lightest hybrid multiplet includes at least one $J^{PC}$ exotic state.
Multiquark are states with a number of quark-antiquark greater than 3. The colour number are always colourless. An example of a recent discovery of $c\overline{c}q\overline{q}$ states is the Y(4260) \cite{4260}. Hybrid states is a wide topic and it is connected to Charmonium and Charm physics, further description will be given in next sections.

\subsection{Charmonium Physics}
Charmonia are charm-anticharm ($c\overline{c}$) bound states, like the J/$\Psi$ resonance or his excitations and due their heavy mass ($c$ quark mass is $\sim$ 1.29 GeV) they probe the QCD at different energy scale: from hard region, where the coupling constant is small and can be expanded, to soft region, where non-perturvative effects dominate. 

To predict the proprieties of the charmonia states in these regions, a Non-Relativistic QCD (NRQCD) expansion can be used because $m_c$ is large and the motion of the c quark is smaller than the speed of light ($v^2$ $\sim$ 0.3 by potential model and Lattice simulation \cite{Brambilla}). This method allow to expand the theory in power of v and describe the mesons annihilation decays.

 ((** a cos’altro posso associare a NPQCD? **))

In the region where the coupling constant can be expanded, it is the perturbative NRQCD (pNRQCD) if $mv>>\Lambda_{QCD}$. The system is weakly coupled and the potential of the meson is calculated. 

The next challenge is to interpret the new charmonia states that are discovered. 
The spectrum of the charmonium states is been measured and the narrow resonance below the open-charm threshold is experimentally clear. Otherwise many charmonia states have been theorize but not observed. 

The spectrum of the charmonium states can be described by a $c\overline{c}$ potential model that combines a Coulomb-like term and a linear one for the confinement: the Cornell potential. It is descrived in Eq. $\ref{eq:strgpot1}$ and on the left in Fig. $\ref{fig:fgMesonSpectrum:a}$.

	\begin{equation}
	\label{eq:strgpot1}
		V_0^{c\overline{c}} (r) = - \frac{4}{3} \frac{\alpha_s}{r} + br.
	\end{equation}

A spin dependent term is augmented to better describe the scalar nature of the potential:
	\begin{equation}
	\label{eq:strgpot2}
		V_{spin-dep} = \frac{32\pi\alpha_s}{9m_c^2}\vec{S_c} \cdot \vec{S_{\overline{c}}}  \delta(\vec{x}) + \frac{1}{m_c^2} \left[\left(\frac{2\alpha_s}{r^3} - \frac {b}{2r}\right)\vec{L} \cdot \vec{S} + \frac{4\alpha_s}{r^3} T \right]
	\end{equation}

((** aggiungere qualcosa da corso di Diego per spiegare i potenziali ?**))

The predicted and observed spectrum of $c\overline{c}$ states are shown in fig. \ref{fig:fgMesonSpectrum:b}. The observed states within the $D\overline{D}$ threshold are in a good agreement with the theoretical prediction, below it the situation is more complicated. Some observed resonances don't match the teory and new states are present. 

	\begin{figure}[btp]
		\centering
		\begin{subfigure}[h]{0.4\textwidth}
   			\includegraphics[width=\textwidth]{figure/cornell}
			\caption{}
			\label{fig:fgMesonSpectrum:a}
		\end{subfigure}
		\begin{subfigure}[h]{0.58\textwidth}
   			\includegraphics[width=\textwidth]{figure/Figs_spectrum}
			\caption{}
			\label{fig:fgMesonSpectrum:b}
		\end{subfigure}
   		\caption[QCD potential and meson spectrum]{a) Cornell potential with the Coulomb-like term and a linear one. b) Meson spectrum labeled in J$^{PC}$ states and some radiative and hadronic decays. Dotted line rappresent the energy value of the open-charm production.}
	\label{fig:fgMesonSpectrum}
	\end{figure}

Precision measurement are needed to solve some questions ((**quali?? Servirebbe una citazione**)) related to the low-mass charmonium spectrum and BESIII is playing his role to determinate the masses and the widths of all charmonium states and their partial width.

There are some mesons, charmonium-like states, that have been observed but do not fit the $c\overline{c}$ model discussed previously and other mesons that could exist but they are not totally been observed like charmonium hybrid. 
Particle of interest are XYZ mesons: multiquarks candidates. 
In April 26, 2013 BESIII announce a new mystery particle: Z$_c^+$(3900) the first observation of a tetra-quark or a charm molecule confirmed later by other experiments.

Charmonium spectroscopy is studied with the hadronic and radiative transitions.
Hadronic transitions are decay modes of heavy quarkonia to lighter $c\overline{c}$ state and a light hadron. The typical mass different between the initial and final meson is around few MeV, so that the typical momentum of the emitted hadron is low. The light hadron is produced from gluons emitted in S,D and P-Wave mode. State of interest are $h_c \rightarrow \pi\pi$ transition.

Information about the wave-function of the $1^{--}$ charmonium states is accessible from the leptonic partial widths. In the non-relativistic limit of an S-wave and D-wave quarkonium system the coupling $e^+e^-$ through a virtual photon involves the wavefunction at contact than the partial width is given by \cite{VanRoyen}:

	\begin{equation}
	\label{eq:Width1}
		\Gamma^{e^+e^-}_{c\overline{c}} \left(^3S_1 \right) = \frac{16}{9} \alpha^2 \frac{\left|\psi(0)\right|^2}{M^2_{c\overline{c}}}.
	\end{equation}

	\begin{equation}
	\label{eq:Width2}
		\Gamma^{e^+e^-}_{c\overline{c}} \left(^3D_1 \right) = \frac{50}{9} \alpha^2 \frac{\left|\psi(0)\right|^n}{M^2_{c\overline{c}}m_c^4}.
	\end{equation}

Radiative decay can be used to extract the $\alpha_s\left(M_{J/\Psi}\right)$ from the ratio $\Gamma(J/\Psi \rightarrow \gamma_{direct} X$ ) over $\Gamma_{strong} (J/\Psi \rightarrow X $) where X stands for light hadrons and $\gamma_{direct}$ a photon produced by the J/$\Psi$.
At BESIII a huge data samples of vector charmonium states as J/$\Psi$,$\Psi$’ and $\Psi$ ’’ is produce and it allow to understand the light hadron spectroscopy and charmonium decay dynamics.

Hadronics decays are the 85-98\% of the charmonia mesons, the basic process is the annihilation of the $c\overline{c}$ inside the charmonium to light quarks, gluons or leptons. The energy release in the process is 2mc and the space-time distance is $\sim$ $\frac{1}{2m_c}$. 
J/$\Psi$, $\Psi$’, $\eta_c$ and $\chi_c$ decays to light hadrons are used to test theories as NPQCD and extract the variables of these or to access to the gluonic behaviour.

Other dacays are the open-flavor decays than occur when there is no annihilation of the $c\overline{c}$ pair. Measuring their branching fractions is experimentally challenging.

Due his huge J/$\Psi$ and $\Psi(2S)$ data sample, rare and forbidden charmonium decays are accessible at BESIII experiment. Precise test of the theory and accurate determinations of many parameters of the Standard Model are accessible as the OZI-violating but flavour-conserving decays, invisible decays of quarkonium states, CP violating process and lepton flavour decay.
OZI-violating but flavour-conserving decays are searched in narrow natural width of the J/$\Psi$ and $\Psi$(2S) states. The huge decay samples of J/$\Psi$ allow to find some anomalous production rate that would be an hint of possible new physics.
Through the channel $\Psi \rightarrow D_s^+\pi^-$ ($\Psi \rightarrow D_s^+\rho^-$) Cabibbo allowed (suppressant) decays are tested. Semileptonic decays are used too.

Invisible decays of charmonium states allow to look for new physics.  The neutrino is the only one particle that can not be detected. Light dark matter and new particles can be observed in $\eta$ and $\eta$’ decays.
It has been shown that measurements of the J/$\Psi$ invisible decay widths can be used
to constrain new physics models \cite{LNChang}.

Standard Model lepton-flavor-violating (LFV) processes are suppressed due very small neutrino masses \cite{Nussinov}. BESIII experiment through the channel J/$\Psi$ $\rightarrow$ ll’ (l$\neq$l’) make high sensitivity search for LFV, predicted in SMMS.

\subsection{Charm physics}
D mesons are the lightest particle containing charm quark and due to SM prediction the D system is good to test the theory through their leptonic and semi-leptonic decay to access to the CKM matrix and $D^0\overline{D^0}$ mixing to the CP asymmetries. Also hadronic and rare decays are studied.

The potential used in D meson decays need precise theoretical control to describe branching ratio, spectrum and quantum number of charmed meson as $D^0$, $D^+$, $D_s^0$ and $D_s^+$.

Meanwhile SM predicts small CP-violating asymmetries in charmed particle decay because the mode is Cabibbo suppressed and a large data sample is required with a complex final states to be analyzed.

To produce D mesons via $e^+e^- \rightarrow$ hadrons a $c\overline{c}$ resonance above the D$\overline{D}$ threshold have to be created. There are four broad resonance states that decay into pair of charmed meson final states: the initial $c\overline{c}$ meson decays via the production of light $q\overline{q}$ pair and forms $c\overline{q}$-$\overline{c}q$ system that separate in two charmed mesons. This production mechanism is poorly understood.

These states are the $\Psi$(3770), $\Psi$(4040), $\Psi$(4160) and $\Psi$(4415). They are easily produced at $e^+e^-$ collider because their quantum number $J^{PC}$ $1^{--}$.
To study this mechanism the charmed cross section is measured
	\begin{equation}
	\label{eq:cross1}
		\sigma_{charm} = \frac{N_{charm}}{\mathcal{L}}.
	\end{equation}

where $\mathcal{L}$ is the integrated luminosity and $N_{charm}$ is the number of charmed meson obtained using tagging technique.

The cross section of the $c\overline{c}$ states above the open-charm threshold can be understood as the successive onset of the charmed meson channels: $D\overline{D}$,$D^*\overline{D}$,$D^*\overline{D^*}$,$D_s\overline{D}_s$, etc...
Each charm decay of these charmonium state is studied to determinate amplitude and width and to compare with the theory that describe these decays \cite{Brambilla}.

Usual decay mode used for tagging are: 

 $D^0 \rightarrow K^- \pi^+ (\sim 4\%)$, $D^0 \rightarrow K^- \pi^+\pi^+\pi^-(\sim 8\%)$, $D^0 \rightarrow K^-\pi^+\pi^0(\sim 14\%)$, $D^+ \rightarrow K^-\pi^+\pi^+$($\sim$ 9\%), $D^+ \rightarrow K^0\pi^+$($\sim$ 3\%), $D^+ \rightarrow K^0\pi^+\pi^0$($\sim$ 14\%), $D^+ \rightarrow K^0\pi^+\pi^+\pi^-$($\sim$ 6\%), $D^+ \rightarrow K^-\pi^+\pi^+\pi^0$($\sim$ 6\%).
PID algorithm is used to identify kaons and pions  to reduce the combinatoric background. Neutral track are identified by the EMC ($e.g.$ $\pi^0\rightarrow\gamma \gamma$).

Other constrain came from the invariant mass ($M_{inv}$) and the beam constrained mass ($M_{bc}$) defined in Eqs. \ref{eq:constain1} and \ref{eq:constain2}:
 	\begin{equation}
	\label{eq:constain1}
		M_{inv}= \sqrt{\left (\sum_i E_i \right )^2 - \left (\sum_i \vec {p}_i \right )^2}.
	\end{equation}

	\begin{equation}
	\label{eq:constain2}
		M_{bc}= \sqrt{E^2_{beam} - \left (\sum_i \vec {p}_i \right )^2} = \sqrt{E^2_{beam} - p_D^2}.
	\end{equation}
Pure leptonic decays $D^+\rightarrow l^+\nu$ are the cleanest decay modes of $D^+$ meson : the $c$ and $\overline{d}$ quarks annihilate into a virtual $W^+$ boson with a decay width give by the SM:

	\begin{equation}
	\label{eq:Width3}
		\Gamma \left (D^+ \rightarrow l^+ \nu \right ) = \frac{G^2_F}{8\pi} f_{D^+}^2 m_l^2 M_{D^+} \left (1 - \frac{m_l^2}{M^2_{D^+}} \right ) |V_{cd}|^2.
	\end{equation}

Where $M_D^+$ is the $D^+$ mass, $m_l$ is the lepton mass, $V_{cd}$ is the CKM matrix element and $f_{D+}$ is the decay constant that contains the information about the dynamics of the quarks inside the meson.
Studying this kind of decay it determines $f_{D+} |V_{cd}|$. In the literature, $f_{D+}$ has been extensively studied in a variety of theoretical approaches \cite{TWChiu,Narison}.

In similar way $D_s^+ \rightarrow l^+ \nu$ mode is used to access to $|V_{cs}|$ and $f_{D_s}$.
BESIII physics program include high precision measurement of $f_D$ and $f_{D_s}$ mesons.

Semileptonic decays occur when a charm meson decay via weak interaction by emitting a $l^+\nu$ lepton pair: $c\rightarrow ql^+\nu$, where q=d,s. The q quark is bound to the initial light quark of the charm meson by strong interaction (X meson in Eq. \ref{eq:Amplitude}). In semileptonic decay the leptons do not interfere with the strong interaction then they can factored out the hadronic process. The process amplitude is: 
	\begin{equation}
	\label{eq:Amplitude}
		\mathcal{A} = \frac{G_F}{\sqrt{2}}V^*_{cq}\overline{\nu}\gamma_{\mu}(1-\gamma_5)l\left \langle  X|\overline{q}\gamma^{\mu}(1-\gamma_5)c|D\right \rangle.
	\end{equation}
The process depend to the quark-mixing parameter $V_{cq}$ so the semileptonic decay is a good system to access to the CKM matrix and test the technique that calculate the hadronic matrix element developed by several method \cite{Abada,Shifman,Khodja,Wirbel,HYCheng,Fajfer}.
These decay are sensitive to $V_{cd}$ and $V_{cs}$ by the determination of the absolute branching fractions, $e.g.$ for $V_{cs}$ in $D \rightarrow \pi l^+ \nu$, $D \rightarrow K l^+\nu$, $D \rightarrow \eta(\eta')l^+\nu$, $D \rightarrow \rho l^+\nu$, $D \rightarrow K^*l^+\nu$, $D_s \rightarrow \varphi l^+\nu$, etc.

These parameter used together with the other CKM element defined in \ref{eq:VCKM} and used to measure the mixing and the CP violating paramenter, to test the self-consistency of the CKM picture, to search possible new physics beyond the CKM mechanism.

	\begin{equation}
	\label{eq:VCKM}
		V_{CKM} = \begin{pmatrix}
V_{ud} & V_{us} & V_{ub}\\ 
V_{cd} & V_{cs} & V_{cb}\\ 
V_{td} & V_{ts} & V_{tb} 
\end{pmatrix}.
	\end{equation}

The CKM matrix is an unitary matrix which contains information on the strength of flavour-changing weak decays. For a 3x3 flavor matrix CP violation can be describe as function of these elements. A parameterization of the 4 independent variable of the $V_{CKM}$ came from the unitary relation  

	\begin{equation}
	\label{eq:CKMunit}
		\sum_k V_{ik}V^*_{jk} = 0
	\end{equation}

((**forse meglio $V_{ud} V_{ub}^* + V_{cd} V_{cb}^* + V_{td} V_{tb}^*$ **))  

that form the unitary triangle. Since the three sides of the triangles are open to direct experiment, as are the three angles, a class of tests of the Standard Model is to check that the triangle closes. 

The state of art of these variable is shown in fig \ref{fig:fgCKM} as function of the $\alpha$, $\beta, \gamma$ angles and $\overline{\eta} - \overline{\rho}$ coordinate.

	\begin{figure}[btp]
		\centering
   		\includegraphics[width=0.8\textwidth]{figure/UnitaryTriangle.pdf}
   		\caption[Unitary triangle.]{The unitary triangle shows the constrain of the CP violation. $\alpha$,$\beta$ and $\gamma$ are the angles, $\overline{\rho}$ and $\overline{\eta}$ the coordinates. They are connected to the CKM matrix. Coloured areas show the experimental constrains of these angles and coordinates \cite{CKM}.}
	\label{fig:fgCKM}
	\end{figure}

The main goal of CP-violating experiments is to over-constrain these parameters to find inconsistency suggesting new physics over the SM.
Further the weak decay, hadronic decay are studied to describe the QCD theory. Charm system allow to access to physics region below $\Lambda_{QCD}$ by light flavour quarks and up to $\Lambda_{QCD}$. LatticeQCD and perturbative theory are tested in decay with two-body and three-body decay. The high number of decay channels give a data sample to test different modes from D meson to pseudoscalar, scalar, vector, axial and tensor mesons.  \\

Meson-antimeson oscillation is another topic accessible at BESIII experiment. In these oscillation weak interaction effect build up over macroscopic distance and makes tiny mass differences measurable. It is mandatory to probe $D^0-\overline{D^0}$ oscillation as sensitively as possible to provide proof of New Physics and CP violation.

Mass eigenstates of quarks are compose by different flavors giving rise to the non-diagonal CKM matrix and a mixing that allow $D^0-\overline{D^0}$ oscillation.

	\begin{figure}[btp]
		\centering
   		\includegraphics[width=0.8\textwidth]{figure/Doscillation.pdf}
   		\caption[$D^0-\overline{D^0}$ oscillation.]{Feyman diagram of the $D^0-\overline{D^0}$ oscillation in s channel (right) and t channel (left) through the exchange of two $W$ bosons.}
	\label{fig:fgDOscillation}
	\end{figure}

The flavour eigenstates $D^0$ and $\overline{D^0}$ are different from the effective Hamiltonian eigenstates $D_1$ and $D_2$ given by:

	\begin{equation}
	\label{eq:Doscillation}
		|D_1 \rangle = \frac{1}{\sqrt{|p|^2+|q|^2}}\left (p|D^0\rangle+q|\overline{D}^0\rangle\right), |D_2 \rangle = \frac{1}{\sqrt{|p|^2+|q|^2}}\left (p|D^0\rangle-q|\overline{D}^0\rangle\right).
	\end{equation}

Schrodinger-like equation describe the time evolution as function of the mass matrix M and decay matrix $\Gamma$. 
There are two interesting dimensionless values that describe the oscillation:

	\begin{equation}
	\label{eq:XandY}
		x\equiv \frac{\Delta m}{\Gamma},y\equiv \frac{\Delta \Gamma}{2\Gamma}.
	\end{equation}

Where $\Delta m$ and $\Delta\Gamma$ is the difference between the mass and decay eigenvalue of the effective Hamiltonian eigenstates. Hadronic and semi-leptonic decays are studied to measure the amplitude $\mathcal{A}(B^0\rightarrow B^0(t))$ and viceversa. D mesons decay into CP final states and their lifetime, strong phase and mixing rate $R_M$ are studied at the $\Psi$(3770) peak. After that CP violation is found in decay, mixing and interference.

((**scrivere meglio sto pezzo?**))\\

Last charm decays searched at BESIII are rare and forbidden decays: SM needs more precise measurement to test it and to find same information about the main physics problem about the mass hierarchy, fine tuning, etc… Potentially interesting decays include: 
\begin{itemize}
\item $D \rightarrow V \gamma(V = \rho, \omega, \varphi, ...)$ , 
\item $D \rightarrow Xl^+l^- (X =\pi,K, \eta, \rho, \omega, \varphi, ...)$, 
\item $D \rightarrow X\nu l^-\nu_l  (X = \pi,K, \eta )$, (iv) $D \rightarrow \gamma\gamma$, and (v) $D \rightarrow l^+l^-$.
\end{itemize}
Other rare decays are searching New Physics as SUSY and extra-dimension.

\subsection{Tau Physics}
An $e^+e^-$ collider running at $\tau$ threshold produce a large sample of tau leptons that decay in a tau neutrino plus hadrons with a branching fraction of 64.8\%.
This channel allow to access at the strange and non-strange spectral function, to chiral perturbation at low $Q^2$, to spectroscopy of light mesons. Hadronic tau decays are a good laboratory for QCD and can determinate $V_{us}$. CP asymmetries are also a available, the most promising channels are $\tau^- \rightarrow \nu_{\tau} K_S\pi^- , \nu_{\tau} K^-\pi^0$.


